DEEP: Edge-based Dataflow Processing with Hybrid Docker Hub and Regional Registries

Reducing energy consumption is essential to lessen greenhouse gas emissions, conserve natural resources, and help mitigate the impacts of climate change. In this direction, edge computing, a complementary technology to cloud computing, extends computational capabilities closer to the data producers, enabling energy-efficient and latency-sensitive service delivery for end users. To properly manage data and microservice storage, expanding the Docker Hub registry to the edge using an AWS S3-compatible MinIO-based object storage service can reduce completion time and energy consumption. To address this, we introduce Docker rEgistry-based Edge dataflow Processing (DEEP) to optimize the energy consumption of microservice-based application deployments by focusing on deployments from Docker Hub and MinIO-based regional registries and their processing on edge devices. After applying nash equilibrium and benchmarking the execution of two compute-intensive machine learning (ML) applications of video and text processing, we compare energy consumption across three deployment scenarios: exclusively from Docker Hub, exclusively from the regional registry, and a hybrid method utilizing both. Experimental results show that deploying 83% of text processing microservices from the regional registry improves the energy consumption by 0.34% (18J) compared to microservice deployments exclusively from Docker Hub.

==> archive.tex <==

% \subsubsection*{Block storage}
% MinIO is an open-source, high-performance distributed object storage platform\footnote{\url{https://github.com/minio/minio}}. It supports cloud object storage technologies such as Amazon Simple Storage Service (S3) and Kubernetes orchestrator, enabling the storage of unstructured data such as multimedia, log files, and container or virtual machine images. %It provides a size from 1 KBs to a maximum of 5 TB for a single object. 
% MinIO organizes objects into buckets, accessible through the HTTP API using access and secret keys.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%Li et al.~\cite{li2020capacity} introduced a caching strategy for heterogeneous storage capacities of edge devices to optimize data retrieval time and overall network performance. This method adapts the cache allocation based on the storage limitations of individual edge devices while ensuring that the most frequently accessed data is stored closer to the users. This strategy improves the efficiency of content delivery by maximizing cache utilization across the network and minimizing reliance on distant cloud servers.
%Tran et al.~\cite{tran2017collaborative} proposed an online collaborative joint caching and processing in mobile edge computing (MEC) for multi-bitrate video streaming. In this method, the required bitrate video for a user is produced by the MEC servers collaboration, or a required bitrate video from a cached video is retrieved. This method formulates the caching and processing problem as an integer linear programming that minimizes the network cost incurred when the cache server retrieves a video from another cache server or the origin media server.

% \paragraph{Dataflow transmission time} $T_c\left(m_u,m_i \right)$ of a dataflow $\Data_{ui}$ from a microservice $m_u$ scheduled on $d_k= \sched\left(m_u\right)$ to a microservice $m_i$ scheduled on a device $d_j$ is the sum of its data element transmission times:
% \begin{equation*}
% T_c\left(m_u,m_i\right) = \frac{\SIZE_{ui}}{\BW_{kj}}.
% \end{equation*}
% \paragraph{Deployment time} 
% $T_d(m_i,d_j)$ consists of the time needed to download the containerized microservice image not existing on a device $d_j$%, and its startup %the startup time of the container
% ~\cite{nardelli2017elastic}:
% \begin{equation*}
%     T_d\left(m_i,d_j\right) = \frac{\mathtt{sizeof}(m_i)}{\BW_{j}},
%     \label{eq:deptime}
% \end{equation*}
% where $\mathtt{sizeof}(m_i)$ is size of %the container
% microservice's image stored in a repository (remote or regional), transferred through a bandwidth of $\BW_{j}$ to a device $d_j$ for deployment.


\begin{table}%[!t]
\centering
\caption{Benchmarks of case study applications (images on Docker Hub and $\dcloudID$) on Lenovo device.}
\label{tbl:bechmark:dep+exec+docker+hub}
\resizebox{\columnwidth}{!}
{ 
\begin{tabular}{|cccccc|}
\cline{2-4}
\multicolumn{1}{c}{} &\multicolumn{1}{|c|}{\textit{Microservice}}       & \multicolumn{1}{c|}{$T_p$ [\si{\second}] }  &\multicolumn{1}{c|}{$\ec$ [\si{\joule}]}   %& \multicolumn{1}{c|}{CPU\_energy [\si{\joule}]}     & \multicolumn{1}{c|}{MEM\_energy [\si{\joule}]} 
\\ \hline
 \multirow{6}{.9cm}{\centering {\rotatebox[origin=c]{90}{\makecell{{{\textit{Video}}}\\{{\textit{processing}}}\\ {{\textit{application}}}}}}}&\multicolumn{1}{|c|}{\textit{Transcode}} & \multicolumn{1}{c|}{17.5--19.1}   & \multicolumn{1}{c|}{856.5--859} &\multicolumn{1}{c|}{82--85}   & \multicolumn{1}{c|}{340--355}&\multicolumn{1}{c|}{0.17} 
 \\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{Frame}}               & \multicolumn{1}{c|}{9.6--20.2} & \multicolumn{1}{c|}{354.31--377.4} 
& \multicolumn{1}{c|}{147--184} & \multicolumn{1}{c|}{557--679} & \multicolumn{1}{c|}{0.70}
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Train}}           & \multicolumn{1}{c|}{12.6--123.9} & \multicolumn{1}{c|}{3239.5--3288.3} 
&\multicolumn{1}{c|}{5.78} &\multicolumn{1}{c|}{1071--1421} & \multicolumn{1}{c|}{4654--5472}  
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Train}}           & \multicolumn{1}{c|}{87.2--96.6}&  \multicolumn{1}{c|}{1833.5--1848.7} 
%& \multicolumn{1}{c|}{1761.5}     & \multicolumn{1}{c|}{72.0}   
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Infer}}          & \multicolumn{1}{c|}{38--40.8} & \multicolumn{1}{c|}{848.7--850.1} 
%&\multicolumn{1}{c|}{821.03} & \multicolumn{1}{c|}{27.69}     
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Infer}}          & \multicolumn{1}{c|}{38.2--44} & \multicolumn{1}{c|}{819--841.6}
%&\multicolumn{1}{c|}{789.5} & \multicolumn{1}{c|}{29.5}    
\\
\hline
\multirow{6}{.9cm}{\centering {\rotatebox[origin=c]{90}{\makecell{{{\textit{Text}}} \\{{\textit{processing}}}\\{{\textit{application}}}}}}}&\multicolumn{1}{|c|}{\textit{Retrieve}}  & \multicolumn{1}{c|}{42.3--58.1}  & \multicolumn{1}{c|}{143.5--172.4}  
%& \multicolumn{1}{c|}{139.53}  & \multicolumn{1}{c|}{32.9}
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{Decompress}} &  \multicolumn{1}{c|}{26.9--54.6} & \multicolumn{1}{c|}{415--431.9} 
%&\multicolumn{1}{c|}{383.85}   & \multicolumn{1}{c|}{31.15}   
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Train}}           & \multicolumn{1}{c|}{138.8--143.7} & \multicolumn{1}{c|}{3481.7--3727.8}    
%& \multicolumn{1}{c|}{3388.63}   & \multicolumn{1}{c|}{93.08}   
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Train}}           &  \multicolumn{1}{c|}{86.5--88.9} & \multicolumn{1}{c|}{1621.8--1641.6}   
%& \multicolumn{1}{c|}{1571.95}   & \multicolumn{1}{c|}{49.8} 
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Score}}               & \multicolumn{1}{c|}{73.4--75.5} & \multicolumn{1}{c|}{1227.5--1319.3}   
%& \multicolumn{1}{c|}{1187.21}        & \multicolumn{1}{c|}{40.31}     
\\\cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Score}}           &  \multicolumn{1}{c|}{74.5--77.6}  & \multicolumn{1}{c|}{1295.5--1298.7}  
%& \multicolumn{1}{c|}{1255.72}   & \multicolumn{1}{c|}{43.01}  
\\ 
\hline
\end{tabular}}
\end{table}

%
% 
% 
%\multicolumn{1}{c|}{5.78} & \multicolumn{1}{c|}{0}&  \multicolumn{1}{c|}{0} &  
%\multicolumn{1}{c|}{3.53} & \multicolumn{1}{c|}{356--435} & \multicolumn{1}{c|}{1423--1602} &
%\multicolumn{1}{c|}{3.54} & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0} &
%\multicolumn{1}{c|}{0.14} & \multicolumn{1}{c|}{331--334}  & \multicolumn{1}{c|}{1136--1183}  &
%\multicolumn{1}{c|}{0.78}& \multicolumn{1}{c|}{290--331} & \multicolumn{1}{c|}{1037--1143} &
%\multicolumn{1}{c|}{2.36}&\multicolumn{1}{c|}{427--507} & \multicolumn{1}{c|}{1638--1903} &
%\multicolumn{1}{c|}{2.36} & \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0}  &
%\multicolumn{1}{c|}{0.63} & \multicolumn{1}{c|}{177--211} & \multicolumn{1}{c|}{675--786} & 
%\multicolumn{1}{c|}{0.63}  &  \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0}  &


% \begin{table*}[!t]
% \centering
% \caption{Case study applications' energy benchmarks (images on $\dcloudID$ Docker Hub).}
% \label{tbl:bechmark:edp+exec+aau+hub}
% \resizebox{\columnwidth}{!}
% { 
% \begin{tabular}{|ccccc|}
% \cline{2-4}
% \multicolumn{1}{c}{} &\multicolumn{1}{|c|}{Microservice}              & \multicolumn{1}{c|}{$\ct$ [\si{\second}] }  &\multicolumn{1}{c|}{$\ec$ [\si{\joule}]}   %& \multicolumn{1}{c|}{CPU\_energy [\si{\joule}]}     & \multicolumn{1}{c|}{MEM\_energy [\si{\joule}]} 
% \\ \hline
%  \multirow{6}{.9cm}{\centering {\rotatebox[origin=c]{90}{\makecell{{{Video}}\\{{processing}}\\ {{application}}}}}}&\multicolumn{1}{|c|}{\textit{Transcode}} & \multicolumn{1}{c|}{17.5} &  \multicolumn{1}{c|}{856.5}
%  %& \multicolumn{1}{c|}{834.4}   & \multicolumn{1}{c|}{22.1} 
%  \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{Frame}}               & \multicolumn{1}{c|}{19.6}& \multicolumn{1}{c|}{377.4} %& \multicolumn{1}{c|}{361.2}   & \multicolumn{1}{c|}{16.2}  
% \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{HA Train}}           & \multicolumn{1}{c|}{112.6}& \multicolumn{1}{c|}{3239.5}  %& \multicolumn{1}{c|}{3114.5}     & \multicolumn{1}{c|}{125.0}   
% \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{LA Train}}           & \multicolumn{1}{c|}{87.2} &\multicolumn{1}{c|}{1848.7}  %& \multicolumn{1}{c|}{1783.4}     & \multicolumn{1}{c|}{65.3}   
% \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{HA Infer}}          & \multicolumn{1}{c|}{38.0} & \multicolumn{1}{c|}{850.1}
% %& \multicolumn{1}{c|}{824.2} & \multicolumn{1}{c|}{25.9}   
% \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{LA Infer}}          & \multicolumn{1}{c|}{38.2} & \multicolumn{1}{c|}{841.6}
% %& \multicolumn{1}{c|}{815.9} & \multicolumn{1}{c|}{25.7}    
% \\ \cline{2-4} \hline

%  \multirow{6}{.9cm}{\centering {\rotatebox[origin=c]{90}{\makecell{{{Text}} \\{{processing}}\\{{application}}}}}}&\multicolumn{1}{|c|}{\textit{Retrieve}}  & \multicolumn{1}{c|}{42.3} & \multicolumn{1}{c|}{143.5}   
%  %& \multicolumn{1}{c|}{119.3}        & \multicolumn{1}{c|}{24.2}
%  \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{Decompress}}             &  \multicolumn{1}{c|}{26.9} & \multicolumn{1}{c|}{431.9}
% %& \multicolumn{1}{c|}{415.6}   & \multicolumn{1}{c|}{16.3}  
% \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{HA Train}}           & \multicolumn{1}{c|}{143.7} & \multicolumn{1}{c|}{3727.8}    %& \multicolumn{1}{c|}{3631.2}   & \multicolumn{1}{c|}{96.6}  
% \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{LA Train}}           &  \multicolumn{1}{c|}{86.5}    & \multicolumn{1}{c|}{1641.6}
% %& \multicolumn{1}{c|}{1593.2}   & \multicolumn{1}{c|}{48.4} 
% \\ \cline{2-4}
% &\multicolumn{1}{|c|}{\textit{HA Score}}               & \multicolumn{1}{c|}{75.5}   & \multicolumn{1}{c|}{1319.3}
% %& \multicolumn{1}{c|}{1277.2}        & \multicolumn{1}{c|}{42.1}     
% \\\cline{2-4}
% &\multicolumn{1}{|c|}{\textit{LA Score}}           &  \multicolumn{1}{c|}{74.7}  & \multicolumn{1}{c|}{1298.7}  %& \multicolumn{1}{c|}{1254.6}   & \multicolumn{1}{c|}{40.9}  
% \\ 
% \hline
% \end{tabular}}
% \end{table*}

\begin{table}%[!t]
\centering
\caption{Benchmarks of case study applications (images on Docker Hub and $\dcloudID$) on the RPi4.}
\label{tbl:bechmark:dep+exec+docker+hub}
\resizebox{\columnwidth}{!}
{ 
\begin{tabular}{|cccc|}
\cline{2-4}
\multicolumn{1}{c}{} &\multicolumn{1}{|c|}{\textit{Microservice}}       & \multicolumn{1}{c|}{$\ct$ [\si{\second}] }  &\multicolumn{1}{c|}{$\ec$ [\si{\joule}]}   %& \multicolumn{1}{c|}{CPU\_energy [\si{\joule}]}     & \multicolumn{1}{c|}{MEM\_energy [\si{\joule}]} 
\\ \hline
 \multirow{6}{.9cm}{\centering {\rotatebox[origin=c]{90}{\makecell{{{\textit{Video}}}\\{{\textit{processing}}}\\ {{\textit{application}}}}}}}&\multicolumn{1}{|c|}{\textit{Transcode}} & \multicolumn{1}{c|}{82--85}   & \multicolumn{1}{c|}{340--355}
 %&\multicolumn{1}{c|}{836.02}   & \multicolumn{1}{c|}{23.01} 
 \\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{Frame}}               & \multicolumn{1}{c|}{147--184} & \multicolumn{1}{c|}{557--679} 
%& \multicolumn{1}{c|}{337.51}   & \multicolumn{1}{c|}{16.84}
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Train}}           & \multicolumn{1}{c|}{1071--1421} & \multicolumn{1}{c|}{4654--5472} 
%& \multicolumn{1}{c|}{3156.01}   & \multicolumn{1}{c|}{132.31}   
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Train}}           & \multicolumn{1}{c|}{0}&  \multicolumn{1}{c|}{0} 
%& \multicolumn{1}{c|}{1761.5}     & \multicolumn{1}{c|}{72.0}   
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Infer}}          & \multicolumn{1}{c|}{356--435} & \multicolumn{1}{c|}{1423--1602} 
%&\multicolumn{1}{c|}{821.03} & \multicolumn{1}{c|}{27.69}     
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Infer}}          & \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0}
%&\multicolumn{1}{c|}{789.5} & \multicolumn{1}{c|}{29.5}    
\\
\hline
\multirow{6}{.9cm}{\centering {\rotatebox[origin=c]{90}{\makecell{{{\textit{Text}}} \\{{\textit{processing}}}\\{{\textit{application}}}}}}}&\multicolumn{1}{|c|}{\textit{Retrieve}}  & \multicolumn{1}{c|}{331--334}  & \multicolumn{1}{c|}{1136--1183}  
%& \multicolumn{1}{c|}{139.53}  & \multicolumn{1}{c|}{32.9}
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{Decompress}} &  \multicolumn{1}{c|}{290--331} & \multicolumn{1}{c|}{1037--1143} 
%&\multicolumn{1}{c|}{383.85}   & \multicolumn{1}{c|}{31.15}   
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Train}}           & \multicolumn{1}{c|}{427--507} & \multicolumn{1}{c|}{1638--1903}    
%& \multicolumn{1}{c|}{3388.63}   & \multicolumn{1}{c|}{93.08}   
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Train}}           &  \multicolumn{1}{c|}{0} & \multicolumn{1}{c|}{0}   
%& \multicolumn{1}{c|}{1571.95}   & \multicolumn{1}{c|}{49.8} 
\\ \cline{2-4}
&\multicolumn{1}{|c|}{\textit{HA Score}}               & \multicolumn{1}{c|}{177--211} & \multicolumn{1}{c|}{675--786}   
%& \multicolumn{1}{c|}{1187.21}        & \multicolumn{1}{c|}{40.31}     
\\\cline{2-4}
&\multicolumn{1}{|c|}{\textit{LA Score}}           &  \multicolumn{1}{c|}{0}  & \multicolumn{1}{c|}{0}  
%& \multicolumn{1}{c|}{1255.72}   & \multicolumn{1}{c|}{43.01}  
\\ 
\hline
\end{tabular}}
\end{table}
\pgfplotstableset{
    /color cells/min/.initial=0,
    /color cells/max/.initial=1000,
    /color cells/textcolor/.initial=,
    %
    % Usage: 'color cells={min=<value which is mapped to lowest color>, 
    %   max = <value which is mapped to largest>}
    color cells/.code={%
        \pgfqkeys{/color cells}{#1}%
        \pgfkeysalso{%
            postproc cell content/.code={%
                %
                \begingroup
                %
                % acquire the value before any number printer changed
                % it:
                \pgfkeysgetvalue{/pgfplots/table/@preprocessed cell content}\value
                \ifx\value\empty
                    \endgroup
                \else
                \pgfmathfloatparsenumber{\value}%
                \pgfmathfloattofixed{\pgfmathresult}%
                \let\value=\pgfmathresult
                %
                % map that value:
                \pgfplotscolormapaccess
                    [\pgfkeysvalueof{/color cells/min}:\pgfkeysvalueof{/color cells/max}]
                    {\value}
                    {\pgfkeysvalueof{/pgfplots/colormap name}}%
                % now, \pgfmathresult contains {<R>,<G>,<B>}
                % 
                % acquire the value AFTER any preprocessor or
                % typesetter (like number printer) worked on it:
                \pgfkeysgetvalue{/pgfplots/table/@cell content}\typesetvalue
                \pgfkeysgetvalue{/color cells/textcolor}\textcolorvalue
                %
                % tex-expansion control
                % see https://tex.stackexchange.com/questions/12668/where-do-i-start-latex-programming/27589#27589
                \toks0=\expandafter{\typesetvalue}%
                \xdef\temp{%
                    \noexpand\pgfkeysalso{%
                        @cell content={%
                            \noexpand\cellcolor[rgb]{\pgfmathresult}%
                            \noexpand\definecolor{mapped color}{rgb}{\pgfmathresult}%
                            \ifx\textcolorvalue\empty
                            \else
                                \noexpand\color{\textcolorvalue}%
                            \fi
                            \the\toks0 %
                        }%
                    }%
                }%
                \endgroup
                \temp
                \fi
            }%
        }%
    }
}
% \pgfplotstabletypeset[
%     color cells={min=0,max=100,textcolor=-mapped color!80!black},
%     /pgfplots/colormap/greenyellow
% ]
% {
%     %$\dcloudID$   $\DockerHubID$   
%     %a         b
%     17    83     
%     0.00   0.00
% }

% \pgfplotstabletypeset[
%     color cells={min=0,max=100,textcolor=-mapped color!80!black},
%     /pgfplots/colormap/greenyellow
% ]
% {
%     %$\dcloudID$   $\DockerHubID$   
%     %a         b
%     17    17     
%     66   0.00
% }
